Lexicographic Ranking Supermartingales with Lazy Lower Bounds

Lexicographic Ranking SuperMartingale (LexRSM) is a probabilistic extension of Lexicographic Ranking Function (LexRF), which is a widely accepted technique for verifying program termination. In this paper, we are the first to propose sound probabilistic extensions of LexRF with a weaker non-negativity condition, called single-component (SC) non-negativity. It is known that such an extension, if it exists, will be nontrivial due to the intricacies of the probabilistic circumstances. Toward the goal, we first devise the notion of fixability, which offers a systematic approach for analyzing the soundness of possibly negative LexRSM. This notion yields a desired extension of LexRF that is sound for general stochastic processes. We next propose another extension, called Lazy LexRSM, toward the application to automated verification; it is sound over probabilistic programs with linear arithmetics, while its subclass is amenable to automated synthesis via linear programming. We finally propose a LexRSM synthesis algorithm for this subclass, and perform experiments.

==> figures/alg.tex <==
\begin{algorithm}[t]
%\small
   \caption{synthesis algorithm of linear SC-LexRSM map with MCLC.}\label{alg:Alg1}
   \textbf{Input:} A pCFG $\mathcal{C}$ with an invariant $I$\;
   Initialize $U\leftarrow $ all generalized transitions of pCFG $\mathcal{C}$\,; $d \leftarrow 0$\;
   \While{$U$ is not empty}{
     $d \leftarrow d+1$;$ranked \leftarrow False$\;
     Construct and solve $\mathcal{LP}^1_U$\;\label{line:consLP1}
     \If{No solution to $\mathcal{LP}^1_U$}{\label{line:IfNoSol}
        \For{each $\calT \in \mbox{Class}(U)$}{\label{line:chooseTransitionsToRank}
            Construct and solve $\mathcal{LP}^2_{U,\calT}$\;
            \If{Exist solution to $\mathcal{LP}^2_{U,\calT}$}{
                $\eta_d \leftarrow $ RF from Solution of $\mathcal{LP}^2_{U,\calT}$;$ranked \leftarrow True$\;\label{line:solvedsingle}
                $U \leftarrow U \backslash \calT$\;\label{line:delsingle}
                break\;\label{line:break}
            }
        }
        \If{not $ranked$}{\label{line:ifnosingle}
            {\bf Return} FALSE\;\label{line:fail}
            }
    }
     \Else{
         $\eta_d \leftarrow $ ranking function from Solution of $\mathcal{LP}^1_U$\;\label{line:solved}
         $U \leftarrow U \backslash \{\tau \mid \eta_d \mbox{ ranks $\tau$}\}$\;\label{line:del}
     }
   }
   {\bf Return} $(\eta_1,\eta_2,\cdots,\eta_d)$
\end{algorithm}

==> figures/fig2_translation_pcfg.tex <==
\tikzstyle{circ}=[shape=circle,draw,inner sep=0pt,minimum size=8mm]
\tikzstyle{circshad}=[shape=circle,draw,inner sep=0pt,minimum size=5mm,fill=gray!20]
\tikzstyle{tran}=[draw,->,>=stealth, rounded corners]


\begin{figure}[!tb]
% \small
\centering
    \subfloat[skip]{\label{fig:PPtoPCFG_skip}
    \begin{minipage}[t]{0.3\linewidth}
    \scalebox{1}{
        \begin{tikzpicture}[x = 2cm]
                \node[circ] (0) at(0,-0.5) {$\ell_{i}$};
                \node[circ] (1) at(1.5,-0.5) {$\ell_{o}$};
                \draw[->] (0)--node[above]{\footnotesize$~\tau: true, 1, id~$} (1);
                % \draw[tran](0) to node[font=\scriptsize,draw, fill=white, rectangle,pos=0.5] {$x \leq 0$} (1);
        \end{tikzpicture}
    }
    \end{minipage}
    }
    \subfloat[$x_i := \langle \mathit{assgn} \rangle$]{\label{fig:PPtoPCFG_assgn}
    \begin{minipage}[t]{0.3\linewidth}
    \scalebox{1}{
    \begin{tikzpicture}[x = 2cm]
            \node[circ] (0) at(0,-0.5) {$\ell_{i}$};
            \node[circ] (1) at(1.5,-0.5) {$\ell_{o}$};
            \draw[->] (0)--node[above]{\footnotesize$~\tau: true, 1, (i,u)$} (1);
            % \draw[tran](0) to node[font=\scriptsize,draw, fill=white, rectangle,pos=0.5] {$x \leq 0$} (1);
    \end{tikzpicture}
    }
    \end{minipage}
    } 
    \subfloat[A;B]{\label{fig:PPtoPCFG_Concatenation}
    \begin{minipage}[t]{0.3\linewidth}
    \scalebox{1}{
    \begin{tikzpicture}[x = 2cm]
            \node[circ,align=center] (0) at(0,-0.5) {$\ell_{i}=$ \\ $\ell^A_{i}$};
            \node[circ,align=center] (1) at(0.8,0) {$\ell^A_{o}=$ \\ $\ell^B_{i}$};
            \node[circ,align=center] (2) at(1.6,-0.5) {$\ell_{o}=$ \\ $\ell^B_{o}$};
            \draw[dotted] (0)--node[above]{~} (1);
            \draw[dotted] (1)--node[above]{~} (2);
            % \draw[tran](0) to node[font=\scriptsize,draw, fill=white, rectangle,pos=0.5] {$x \leq 0$} (1);
    \end{tikzpicture}
    }
    \end{minipage}
    }  
    
    
    \subfloat[if $\varphi$ then A else B]{\label{fig:PPtoPCFG_IfGuard}
    \begin{minipage}[t]{0.45\linewidth}
    \scalebox{1}{
    \begin{tikzpicture}[x = 2cm]
            \node[circ] (0) at(0,-0.5) {$\ell_{i}$};
            \node[circ] (1) at(1.5,-1.5) {$\ell^A_{i}$};
            \node[circ] (2) at(1.5,0.5) {$\ell^B_{i}$};
            \node[circ,align=center] (3) at(2.3,-0.5) {$\ell_{o}=$\\ $\ell^A_{o}=$ \\ $ \ell^B_{o}$};
            \draw[->] (0)--node[above]{~} (1);
            \draw[->] (0)--node[above]{~} (2);
            \draw[dotted] (2)--node[above]{~} (3);
            \draw[dotted] (1)--node[above]{~} (3);
            \node at(0.6,0.4) {\footnotesize$\tau_2:\neg\varphi,1,id$};
            \node at(0.6,-1.4) {\footnotesize$\tau_1:\varphi,1,id$};
            % \draw[tran](0) to node[font=\scriptsize,draw, fill=white, rectangle,pos=0.5] {$x \leq 0$} (1);
    \end{tikzpicture}
    }
    \end{minipage}
    }  
    \subfloat[if $prob(p)$ then A else B]{\label{fig:PPtoPCFG_IfProb}
    \begin{minipage}[t]{0.45\linewidth}
    \scalebox{1}{
    \begin{tikzpicture}[x = 2cm]
            \node[circ] (0) at(0,-0.5) {$\ell_{i}$};
            \node[circ] (1) at(1.5,-1.5) {$\ell^A_{i}$};
            \node[circ] (2) at(1.5,0.5) {$\ell^B_{i}$};
            \node[circ,align=center] (3) at(2.3,-0.5) {$\ell_{o}=$\\ $\ell^A_{o}=$ \\ $ \ell^B_{o}$};
            \draw[->] (0)--node[above]{~} (1);
            \draw[->] (0)--node[above]{~} (2);
            \draw[dotted] (2)--node[above]{~} (3);
            \draw[dotted] (1)--node[above]{~} (3);
            \node at(0.6,0.5) {\footnotesize$\tau:true,1-p,id$};
            \node at(0.6,-1.5) {\footnotesize$\tau:true,p,id$};
            % \draw[tran](0) to node[font=\scriptsize,draw, fill=white, rectangle,pos=0.5] {$x \leq 0$} (1);
    \end{tikzpicture}
    }
    \end{minipage}
    }
    
    \subfloat[if * then A else B]{\label{fig:PPtoPCFG_IfStar}
    \begin{minipage}[t]{0.45\linewidth}
    \scalebox{1}{
    \begin{tikzpicture}[x = 2cm]
\node[circ] (0) at(0,-0.5) {$\ell_{i}$};
            \node[circ] (1) at(1.5,-1.5) {$\ell^A_{i}$};
            \node[circ] (2) at(1.5,0.5) {$\ell^B_{i}$};
            \node[circ,align=center] (3) at(2.3,-0.5) {$\ell_{o}=$\\ $\ell^A_{o}=$ \\ $ \ell^B_{o}$};
            \draw[->] (0)--node[above]{~} (1);
            \draw[->] (0)--node[above]{~} (2);
            \draw[dotted] (2)--node[above]{~} (3);
            \draw[dotted] (1)--node[above]{~} (3);
            \node at(0.6,0.4) {\footnotesize$\tau_2:true,1,id$};
            \node at(0.6,-1.4) {\footnotesize$\tau_1:true,1,id$};
            % \draw[tran](0) to node[font=\scriptsize,draw, fill=white, rectangle,pos=0.5] {$x \leq 0$} (1);
    \end{tikzpicture}
    }
    \end{minipage}
    }
    \subfloat[while $\varphi$ do A od]{\label{fig:PPtoPCFG_while}
    \begin{minipage}[t]{0.45\linewidth}
    \scalebox{1}{
    \begin{tikzpicture}[x = 2cm]
            \node[circ,align=center] (0) at(0,-0.5) {$\ell_{i}=$ \\ $\ell^A_{o}$};
            \node[circ] (1) at(1.7,0.5) {$\ell^A_{i}$};
            \node[circ] (2) at(1.7,-1.5) {$\ell_{o}$};
            \node (dot_beg) at(1.6,0.8)  {~};
            \node (dot_end) at(0.0,-0.1)  {~};
            \draw[->] (0)--node[above]{~} (1);
            \draw[->] (0)--node[above]{~} (2);
            \draw[dotted] (dot_beg)--node[above]{~} (dot_end);
            \node at(1.0,-0.3) {\footnotesize$\tau_1:\varphi,1,id$};
            \node at(0.7,-1.4) {\footnotesize$\tau_2:\neg\varphi,1,id$};
            % \draw[tran](0) to node[font=\scriptsize,draw, fill=white, rectangle,pos=0.5] {$x \leq 0$} (1);
    \end{tikzpicture}
    }
    \end{minipage}
    }
    % \subfloat[if * then A else B]{
    % \begin{minipage}{0.3\linewidth}
    % \begin{tikzpicture[x = 2cm]
    %         \node[circ] (0) at(0,-0.5) {$l_{i}$};
    %         \node[circ] (1) at(1.5,-1) {$l^A_{i}$};
    %         \node[circ] (2) at(1.5,0.5) {$l^B_{i}$};
    %         \node[circ,align=center] (3) at(3,-0.5) {$l_{o}=$\\ $l^A_{o}=$ \\ $ l^B_{o}$};
    %         \draw[->] (0)--node[above]{$\tau_1:true,1,id$} (1);
    %         \draw[->] (0)--node[above]{$\tau_2:true,1,id$} (2);
    %         \draw[->] (2)--node[above]{~} (3);
    %         \draw[->] (1)--node[above]{~} (3);
    %         % \draw[tran](0) to node[font=\scriptsize,draw, fill=white, rectangle,pos=0.5] {$x \leq 0$} (1);
    % \end{tikzpicture}
    % \end{minipage}
    % }
\caption{A translation of PPs into pCFGs. %In the figure, 
Circles $\ell_i$ and $\ell_o$ represent the initial and final locations of the translated pCFG, respectively.
The description ``$\tau:\varphi,p,(i,u)$'' on an arrow from $\ell$ to $\ell'$ shows that the pCFG has a transition $\tau = (\ell,\delta)$ such that $G(\tau) \equiv \varphi$, $\delta(\ell') = p$ and $\myup(\tau) = (i,u)$, where $u$ corresponds to the content of $\langle \mathit{assgn} \rangle$ in the case (b); 
and $\mathit{id} \equiv (1,\lambda \boldsymbol{x}. x_1)$ represents ``no update''.
% The \emph{identity update} $(1,\lambda \boldsymbol{x}. x_1)$, i.e. the one that performs no update, is denoted by $\mathit{id}$. 
Circles $\ell_i^A$ and $\ell_o^A$ represent the initial and final locations of the pCFG for program fragment $A$, whose transitions are abstractly shown by a dotted arrow. the pCFG for $B$ is described similarly.}
\label{fig:PPtoPCFG}	
\end{figure}


==> tables/long-table-129.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{longtable}[]{|lcc|cccccccc|}
\caption{Full Experiment Result. 
Ticks in ``p.l.'' and ``p.a.'' indicate the benchmark has a probabilistic loop and assignment, respectively. 
In the ``dim.'' column, a number indicates that the algorithm found a LexRSM with that dimension; a cross indicates a failure; $\times$* means the computation is aborted by our experiment platform due to {\it out of memory}; ``N/A'' means we did not run the experiment. The ``time'' column shows the computation time in seconds.}\label{tab:longresult}\\
\hline
\multicolumn{3}{|c|}{\multirow{3}{*}{Benchmark Spec.}}                                                                       & \multicolumn{8}{c|}{Synthesis result}                                                                                                                                                                                   \\ \cline{4-11} 
\multicolumn{3}{|c|}{}                                                                                                       & \multicolumn{4}{c|}{Baselines}                                                                                       & \multicolumn{4}{c|}{Our Algs}                                                                    \\ \cline{4-11} 
\multicolumn{3}{|c|}{}                                                                                                       & \multicolumn{2}{c|}{STR}                                  & \multicolumn{2}{c|}{LWN}                                 & \multicolumn{2}{c|}{SMC}                                 & \multicolumn{2}{c|}{EMC}              \\ \hline
\multicolumn{1}{|l|}{Model}                                                             & \multicolumn{1}{c|}{p.l.}  & p.a.  & \multicolumn{1}{c|}{dim.}    & \multicolumn{1}{c|}{time}   & \multicolumn{1}{c|}{dim.}   & \multicolumn{1}{c|}{time}   & \multicolumn{1}{c|}{dim.}   & \multicolumn{1}{c|}{time}   & \multicolumn{1}{c|}{dim.}    & time    \\ \hline
\endfirsthead
\hline
\multicolumn{3}{|c|}{\multirow{3}{*}{Benchmark Spec.}}                                                                       & \multicolumn{8}{c|}{Synthesis result}                                                                                                                                                                                   \\ \cline{4-11} 
\multicolumn{3}{|c|}{}                                                                                                       & \multicolumn{4}{c|}{Baselines}                                                                                       & \multicolumn{4}{c|}{Our Algs}                                                                    \\ \cline{4-11} 
\multicolumn{3}{|c|}{}                                                                                                       & \multicolumn{2}{c|}{STR}                                  & \multicolumn{2}{c|}{LWN}                                 & \multicolumn{2}{c|}{SMC}                                 & \multicolumn{2}{c|}{EMC}              \\ \hline
\multicolumn{1}{|l|}{Model}                                                             & \multicolumn{1}{c|}{p.l.}  & p.a.  & \multicolumn{1}{c|}{dim.}    & \multicolumn{1}{c|}{time}   & \multicolumn{1}{c|}{dim.}   & \multicolumn{1}{c|}{time}   & \multicolumn{1}{c|}{dim.}   & \multicolumn{1}{c|}{time}   & \multicolumn{1}{c|}{dim.}    & time    \\ \hline
\endhead
\multicolumn{1}{|l|}{aaron2}                                                            & \multicolumn{1}{c|}{$\times$} & $\times$ & \multicolumn{1}{c|}{2}      & \multicolumn{1}{c|}{0.12}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.05}   & \multicolumn{1}{c|}{2}      & 0.06    \\ \hline
\multicolumn{1}{|l|}{aaron2}                                                            & \multicolumn{1}{c|}{$\surd$}  & $\times$ & \multicolumn{1}{c|}{2}      & \multicolumn{1}{c|}{0.05}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{2}      & 0.06    \\ \hline
\multicolumn{1}{|l|}{aaron2}                                                            & \multicolumn{1}{c|}{$\surd$}  & $\surd$  & \multicolumn{1}{c|}{2}      & \multicolumn{1}{c|}{0.05}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.05}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{2}      & 0.06    \\ \hline
\multicolumn{1}{|l|}{alain}                                                             & \multicolumn{1}{c|}{$\times$} & $\times$ & \multicolumn{1}{c|}{2}      & \multicolumn{1}{c|}{0.08}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{2}      & 0.07    \\ \hline
\multicolumn{1}{|l|}{alain}                                                             & \multicolumn{1}{c|}{$\surd$}  & $\times$ & \multicolumn{1}{c|}{2}      & \multicolumn{1}{c|}{0.09}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.11}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.10}   & \multicolumn{1}{c|}{2}      & 0.10    \\ \hline
\multicolumn{1}{|l|}{alain}                                                             & \multicolumn{1}{c|}{$\surd$}  & $\surd$  & \multicolumn{1}{c|}{3}      & \multicolumn{1}{c|}{0.16}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.15}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.17}   & \multicolumn{1}{c|}{3}      & 0.17    \\ \hline
\multicolumn{1}{|l|}{ax}                                                                & \multicolumn{1}{c|}{$\times$} & $\times$ & \multicolumn{1}{c|}{3}      & \multicolumn{1}{c|}{0.08}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{3}      & 0.08    \\ \hline
\multicolumn{1}{|l|}{ax}                                                                & \multicolumn{1}{c|}{$\surd$}  & $\times$ & \multicolumn{1}{c|}{3}      & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.08}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{3}      & 0.08    \\ \hline
\multicolumn{1}{|l|}{ax}                                                                & \multicolumn{1}{c|}{$\surd$}  & $\surd$  & \multicolumn{1}{c|}{3}      & \multicolumn{1}{c|}{0.08}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.08}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.08}   & \multicolumn{1}{c|}{3}      & 0.09    \\ \hline
\multicolumn{1}{|l|}{catmouse}                                                          & \multicolumn{1}{c|}{$\times$} & $\times$ & \multicolumn{1}{c|}{2}      & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.05}   & \multicolumn{1}{c|}{2}      & 0.05    \\ \hline
\multicolumn{1}{|l|}{catmouse}                                                          & \multicolumn{1}{c|}{$\surd$}  & $\times$ & \multicolumn{1}{c|}{2}      & \multicolumn{1}{c|}{0.05}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.05}   & \multicolumn{1}{c|}{2}      & 0.06    \\ \hline
\multicolumn{1}{|l|}{catmouse}                                                          & \multicolumn{1}{c|}{$\surd$}  & $\surd$  & \multicolumn{1}{c|}{2}      & \multicolumn{1}{c|}{0.05}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.05}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.05}   & \multicolumn{1}{c|}{2}      & 0.06    \\ \hline
\multicolumn{1}{|l|}{complex}                                                           & \multicolumn{1}{c|}{$\times$} & $\times$ & \multicolumn{1}{c|}{$\times$}  & \multicolumn{1}{c|}{0.08}   & \multicolumn{1}{c|}{$\times$} & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{7}     & \multicolumn{1}{c|}{0.16}   & \multicolumn{1}{c|}{5}      & 254.03  \\ \hline
\multicolumn{1}{|l|}{complex}                                                           & \multicolumn{1}{c|}{$\surd$}  & $\times$ & \multicolumn{1}{c|}{$\times$}  & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{$\times$} & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{7}     & \multicolumn{1}{c|}{0.20}   & \multicolumn{1}{c|}{5}      & 4300.40 \\ \hline
\multicolumn{1}{|l|}{complex}                                                           & \multicolumn{1}{c|}{$\surd$}  & $\surd$  & \multicolumn{1}{c|}{$\times$}  & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{$\times$} & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.09}   & \multicolumn{1}{c|}{3}      & 281.59  \\ \hline
\multicolumn{1}{|l|}{counterex1a}                                                       & \multicolumn{1}{c|}{$\times$} & $\times$ & \multicolumn{1}{c|}{$\times$}  & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{$\times$} & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{$\times$} & \multicolumn{1}{c|}{0.20}   & \multicolumn{1}{c|}{$\times$}  & 18.38   \\ \hline
\multicolumn{1}{|l|}{counterex1b}                                                       & \multicolumn{1}{c|}{$\times$} & $\times$ & \multicolumn{1}{c|}{3}      & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{3}      & 0.07    \\ \hline
\multicolumn{1}{|l|}{counterex1b}                                                       & \multicolumn{1}{c|}{$\surd$}  & $\times$ & \multicolumn{1}{c|}{3}      & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{3}      & 0.08    \\ \hline
\multicolumn{1}{|l|}{counterex1b}                                                       & \multicolumn{1}{c|}{$\surd$}  & $\surd$  & \multicolumn{1}{c|}{3}      & \multicolumn{1}{c|}{0.08}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.08}   & \multicolumn{1}{c|}{3}      & 0.08    \\ \hline
\multicolumn{1}{|l|}{counterex1c}                                                       & \multicolumn{1}{c|}{$\times$} & $\times$ & \multicolumn{1}{c|}{$\times$}  & \multicolumn{1}{c|}{0.08}   & \multicolumn{1}{c|}{$\times$} & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{$\times$} & \multicolumn{1}{c|}{0.14}   & \multicolumn{1}{c|}{$\times$}  & 3.96    \\ \hline
\multicolumn{1}{|l|}{counterex1c}                                                       & \multicolumn{1}{c|}{$\surd$}  & $\times$ & \multicolumn{1}{c|}{$\times$}  & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{$\times$} & \multicolumn{1}{c|}{0.08}   & \multicolumn{1}{c|}{$\times$} & \multicolumn{1}{c|}{0.17}   & \multicolumn{1}{c|}{$\times$}  & 17.07   \\ \hline
\multicolumn{1}{|l|}{counterex1c}                                                       & \multicolumn{1}{c|}{$\surd$}  & $\surd$  & \multicolumn{1}{c|}{$\times$}  & \multicolumn{1}{c|}{0.08}   & \multicolumn{1}{c|}{$\times$} & \multicolumn{1}{c|}{0.08}   & \multicolumn{1}{c|}{$\times$} & \multicolumn{1}{c|}{0.17}   & \multicolumn{1}{c|}{$\times$}  & 17.43   \\ \hline
\multicolumn{1}{|l|}{cousot9}                                                           & \multicolumn{1}{c|}{$\times$} & $\times$ & \multicolumn{1}{c|}{$\times$}  & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{3}      & 0.07    \\ \hline
\multicolumn{1}{|l|}{cousot9}                                                           & \multicolumn{1}{c|}{$\surd$}  & $\times$ & \multicolumn{1}{c|}{$\times$}  & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{$\times$} & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{4}     & \multicolumn{1}{c|}{0.10}   & \multicolumn{1}{c|}{4}      & 0.17    \\ \hline
\multicolumn{1}{|l|}{easy1}                                                             & \multicolumn{1}{c|}{$\times$} & $\times$ & \multicolumn{1}{c|}{1}      & \multicolumn{1}{c|}{0.05}   & \multicolumn{1}{c|}{1}     & \multicolumn{1}{c|}{0.04}   & \multicolumn{1}{c|}{1}     & \multicolumn{1}{c|}{0.05}   & \multicolumn{1}{c|}{1}      & 0.04    \\ \hline
\multicolumn{1}{|l|}{easy1}                                                             & \multicolumn{1}{c|}{$\surd$}  & $\times$ & \multicolumn{1}{c|}{1}      & \multicolumn{1}{c|}{0.04}   & \multicolumn{1}{c|}{1}     & \multicolumn{1}{c|}{0.05}   & \multicolumn{1}{c|}{1}     & \multicolumn{1}{c|}{0.04}   & \multicolumn{1}{c|}{1}      & 0.05    \\ \hline
\multicolumn{1}{|l|}{easy1}                                                             & \multicolumn{1}{c|}{$\surd$}  & $\surd$  & \multicolumn{1}{c|}{1}      & \multicolumn{1}{c|}{0.05}   & \multicolumn{1}{c|}{1}     & \multicolumn{1}{c|}{0.05}   & \multicolumn{1}{c|}{1}     & \multicolumn{1}{c|}{0.05}   & \multicolumn{1}{c|}{1}      & 0.05    \\ \hline
\multicolumn{1}{|l|}{easy2}                                                             & \multicolumn{1}{c|}{$\times$} & $\times$ & \multicolumn{1}{c|}{2}      & \multicolumn{1}{c|}{0.05}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.05}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.05}   & \multicolumn{1}{c|}{2}      & 0.05    \\ \hline
\multicolumn{1}{|l|}{easy2}                                                             & \multicolumn{1}{c|}{$\surd$}  & $\times$ & \multicolumn{1}{c|}{2}      & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.05}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{2}      & 0.06    \\ \hline
\multicolumn{1}{|l|}{easy2}                                                             & \multicolumn{1}{c|}{$\surd$}  & $\surd$  & \multicolumn{1}{c|}{2}      & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{2}      & 0.06    \\ \hline
\multicolumn{1}{|l|}{exmini}                                                            & \multicolumn{1}{c|}{$\times$} & $\times$ & \multicolumn{1}{c|}{2}      & \multicolumn{1}{c|}{0.05}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.05}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.05}   & \multicolumn{1}{c|}{2}      & 0.06    \\ \hline
\multicolumn{1}{|l|}{exmini}                                                            & \multicolumn{1}{c|}{$\surd$}  & $\times$ & \multicolumn{1}{c|}{2}      & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.05}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{2}      & 0.06    \\ \hline
\multicolumn{1}{|l|}{exmini}                                                            & \multicolumn{1}{c|}{$\surd$}  & $\surd$  & \multicolumn{1}{c|}{2}      & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{2}      & 0.06    \\ \hline
\multicolumn{1}{|l|}{insertsort}                                                        & \multicolumn{1}{c|}{$\times$} & $\times$ & \multicolumn{1}{c|}{3}      & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{3}      & 0.07    \\ \hline
\multicolumn{1}{|l|}{insertsort}                                                        & \multicolumn{1}{c|}{$\surd$}  & $\times$ & \multicolumn{1}{c|}{3}      & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{3}      & 0.08    \\ \hline
\multicolumn{1}{|l|}{insertsort}                                                        & \multicolumn{1}{c|}{$\surd$}  & $\surd$  & \multicolumn{1}{c|}{3}      & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{3}      & 0.07    \\ \hline
\multicolumn{1}{|l|}{loops}                                                             & \multicolumn{1}{c|}{$\times$} & $\times$ & \multicolumn{1}{c|}{$\times$}  & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{$\times$} & \multicolumn{1}{c|}{0.05}   & \multicolumn{1}{c|}{4}     & \multicolumn{1}{c|}{0.09}   & \multicolumn{1}{c|}{3}      & 3.99    \\ \hline
\multicolumn{1}{|l|}{ndecr}                                                             & \multicolumn{1}{c|}{$\times$} & $\times$ & \multicolumn{1}{c|}{2}      & \multicolumn{1}{c|}{0.05}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.05}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.05}   & \multicolumn{1}{c|}{2}      & 0.05    \\ \hline
\multicolumn{1}{|l|}{ndecr}                                                             & \multicolumn{1}{c|}{$\surd$}  & $\times$ & \multicolumn{1}{c|}{2}      & \multicolumn{1}{c|}{0.05}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.05}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.05}   & \multicolumn{1}{c|}{2}      & 0.06    \\ \hline
\multicolumn{1}{|l|}{ndecr}                                                             & \multicolumn{1}{c|}{$\surd$}  & $\surd$  & \multicolumn{1}{c|}{2}      & \multicolumn{1}{c|}{0.05}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.05}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.05}   & \multicolumn{1}{c|}{2}      & 0.06    \\ \hline
\multicolumn{1}{|l|}{nestedLoop}                                                        & \multicolumn{1}{c|}{$\times$} & $\times$ & \multicolumn{1}{c|}{$\times$}  & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{$\times$} & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{$\times$} & \multicolumn{1}{c|}{0.11}   & \multicolumn{1}{c|}{$\times$}  & 263.17  \\ \hline
\multicolumn{1}{|l|}{nestedLoop}                                                        & \multicolumn{1}{c|}{$\surd$}  & $\times$ & \multicolumn{1}{c|}{3}      & \multicolumn{1}{c|}{0.08}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.09}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.09}   & \multicolumn{1}{c|}{3}      & 0.09    \\ \hline
\multicolumn{1}{|l|}{nestedLoop}                                                        & \multicolumn{1}{c|}{$\surd$}  & $\surd$  & \multicolumn{1}{c|}{$\times$}  & \multicolumn{1}{c|}{0.15}   & \multicolumn{1}{c|}{$\times$} & \multicolumn{1}{c|}{0.15}   & \multicolumn{1}{c|}{4}     & \multicolumn{1}{c|}{0.18}   & \multicolumn{1}{c|}{3}      & 535.30  \\ \hline
\multicolumn{1}{|l|}{perfect}                                                           & \multicolumn{1}{c|}{$\times$} & $\times$ & \multicolumn{1}{c|}{3}      & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{3}      & 0.08    \\ \hline
\multicolumn{1}{|l|}{perfect}                                                           & \multicolumn{1}{c|}{$\surd$}  & $\times$ & \multicolumn{1}{c|}{3}      & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{3}      & 0.08    \\ \hline
\multicolumn{1}{|l|}{perfect}                                                           & \multicolumn{1}{c|}{$\surd$}  & $\surd$  & \multicolumn{1}{c|}{3}      & \multicolumn{1}{c|}{0.08}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.08}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.08}   & \multicolumn{1}{c|}{3}      & 0.08    \\ \hline
\multicolumn{1}{|l|}{perfect1}                                                          & \multicolumn{1}{c|}{$\times$} & $\times$ & \multicolumn{1}{c|}{3}      & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{3}      & 0.07    \\ \hline
\multicolumn{1}{|l|}{perfect1}                                                          & \multicolumn{1}{c|}{$\surd$}  & $\times$ & \multicolumn{1}{c|}{3}      & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{3}      & 0.08    \\ \hline
\multicolumn{1}{|l|}{perfect1}                                                          & \multicolumn{1}{c|}{$\surd$}  & $\surd$  & \multicolumn{1}{c|}{3}      & \multicolumn{1}{c|}{0.08}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.08}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.08}   & \multicolumn{1}{c|}{3}      & 0.08    \\ \hline
\multicolumn{1}{|l|}{perfect2}                                                          & \multicolumn{1}{c|}{$\times$} & $\times$ & \multicolumn{1}{c|}{3}      & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{3}      & 0.07    \\ \hline
\multicolumn{1}{|l|}{perfect2}                                                          & \multicolumn{1}{c|}{$\surd$}  & $\times$ & \multicolumn{1}{c|}{3}      & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{3}      & 0.08    \\ \hline
\multicolumn{1}{|l|}{perfect2}                                                          & \multicolumn{1}{c|}{$\surd$}  & $\surd$  & \multicolumn{1}{c|}{$\times$}  & \multicolumn{1}{c|}{0.08}   & \multicolumn{1}{c|}{$\times$} & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{$\times$} & \multicolumn{1}{c|}{0.11}   & \multicolumn{1}{c|}{$\times$}  & 0.20    \\ \hline
\multicolumn{1}{|l|}{random1d}                                                          & \multicolumn{1}{c|}{$\times$} & $\times$ & \multicolumn{1}{c|}{2}      & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.05}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.05}   & \multicolumn{1}{c|}{2}      & 0.06    \\ \hline
\multicolumn{1}{|l|}{random1d}                                                          & \multicolumn{1}{c|}{$\surd$}  & $\times$ & \multicolumn{1}{c|}{2}      & \multicolumn{1}{c|}{0.05}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.05}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{2}      & 0.06    \\ \hline
\multicolumn{1}{|l|}{random1d}                                                          & \multicolumn{1}{c|}{$\surd$}  & $\surd$  & \multicolumn{1}{c|}{2}      & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.05}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{2}      & 0.07    \\ \hline
\multicolumn{1}{|l|}{real2}                                                             & \multicolumn{1}{c|}{$\times$} & $\times$ & \multicolumn{1}{c|}{$\times$}  & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{$\times$} & \multicolumn{1}{c|}{0.05}   & \multicolumn{1}{c|}{$\times$} & \multicolumn{1}{c|}{0.15}   & \multicolumn{1}{c|}{$\times$}  & 66.48   \\ \hline
\multicolumn{1}{|l|}{realbubble}                                                        & \multicolumn{1}{c|}{$\times$} & $\times$ & \multicolumn{1}{c|}{3}      & \multicolumn{1}{c|}{0.08}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{3}      & 0.11    \\ \hline
\multicolumn{1}{|l|}{realbubble}                                                        & \multicolumn{1}{c|}{$\surd$}  & $\times$ & \multicolumn{1}{c|}{3}      & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.08}   & \multicolumn{1}{c|}{3}      & 0.08    \\ \hline
\multicolumn{1}{|l|}{realbubble}                                                        & \multicolumn{1}{c|}{$\surd$}  & $\surd$  & \multicolumn{1}{c|}{3}      & \multicolumn{1}{c|}{0.09}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.08}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.09}   & \multicolumn{1}{c|}{3}      & 0.09    \\ \hline
\multicolumn{1}{|l|}{realheapsort}                                                      & \multicolumn{1}{c|}{$\times$} & $\times$ & \multicolumn{1}{c|}{$\times$}  & \multicolumn{1}{c|}{0.09}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.08}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.09}   & \multicolumn{1}{c|}{3}      & 0.10    \\ \hline
\multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}realheapsort\\ \_step1\end{tabular}}    & \multicolumn{1}{c|}{$\times$} & $\times$ & \multicolumn{1}{c|}{$\times$}  & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{3}      & 0.08    \\ \hline
\multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}realheapsort\\ \_step1\end{tabular}}    & \multicolumn{1}{c|}{$\surd$}  & $\surd$  & \multicolumn{1}{c|}{$\times$}  & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{3}      & 0.08    \\ \hline
\multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}realheapsort\\ \_step2\end{tabular}}    & \multicolumn{1}{c|}{$\times$} & $\times$ & \multicolumn{1}{c|}{1}      & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{1}     & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{1}     & \multicolumn{1}{c|}{0.05}   & \multicolumn{1}{c|}{1}      & 0.06    \\ \hline
\multicolumn{1}{|l|}{realselect}                                                        & \multicolumn{1}{c|}{$\times$} & $\times$ & \multicolumn{1}{c|}{3}      & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{3}      & 0.08    \\ \hline
\multicolumn{1}{|l|}{realselect}                                                        & \multicolumn{1}{c|}{$\surd$}  & $\times$ & \multicolumn{1}{c|}{3}      & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.08}   & \multicolumn{1}{c|}{3}      & 0.08    \\ \hline
\multicolumn{1}{|l|}{realselect}                                                        & \multicolumn{1}{c|}{$\surd$}  & $\surd$  & \multicolumn{1}{c|}{3}      & \multicolumn{1}{c|}{0.09}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.08}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.09}   & \multicolumn{1}{c|}{3}      & 0.10    \\ \hline
\multicolumn{1}{|l|}{realshellsort}                                                     & \multicolumn{1}{c|}{$\times$} & $\times$ & \multicolumn{1}{c|}{1}      & \multicolumn{1}{c|}{0.05}   & \multicolumn{1}{c|}{1}     & \multicolumn{1}{c|}{0.04}   & \multicolumn{1}{c|}{1}     & \multicolumn{1}{c|}{0.05}   & \multicolumn{1}{c|}{1}      & 0.05    \\ \hline
\multicolumn{1}{|l|}{realshellsort}                                                     & \multicolumn{1}{c|}{$\surd$}  & $\times$ & \multicolumn{1}{c|}{1}      & \multicolumn{1}{c|}{0.05}   & \multicolumn{1}{c|}{1}     & \multicolumn{1}{c|}{0.04}   & \multicolumn{1}{c|}{1}     & \multicolumn{1}{c|}{0.05}   & \multicolumn{1}{c|}{1}      & 0.05    \\ \hline
\multicolumn{1}{|l|}{realshellsort}                                                     & \multicolumn{1}{c|}{$\surd$}  & $\surd$  & \multicolumn{1}{c|}{$\times$}  & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{2}      & 0.07    \\ \hline
\multicolumn{1}{|l|}{rsd}                                                               & \multicolumn{1}{c|}{$\times$} & $\times$ & \multicolumn{1}{c|}{$\times$}  & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{$\times$} & \multicolumn{1}{c|}{0.05}   & \multicolumn{1}{c|}{$\times$} & \multicolumn{1}{c|}{0.14}   & \multicolumn{1}{c|}{$\times$}  & 2.66    \\ \hline
\multicolumn{1}{|l|}{rsd}                                                               & \multicolumn{1}{c|}{$\surd$}  & $\times$ & \multicolumn{1}{c|}{$\times$}  & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{$\times$} & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{$\times$} & \multicolumn{1}{c|}{0.16}   & \multicolumn{1}{c|}{$\times$}  & 10.57   \\ \hline
\multicolumn{1}{|l|}{rsd}                                                               & \multicolumn{1}{c|}{$\surd$}  & $\surd$  & \multicolumn{1}{c|}{1}      & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{1}     & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{1}     & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{1}      & 0.07    \\ \hline
\multicolumn{1}{|l|}{serpent}                                                           & \multicolumn{1}{c|}{$\times$} & $\times$ & \multicolumn{1}{c|}{$\times$}  & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{$\times$} & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.08}   & \multicolumn{1}{c|}{3}      & 30.59   \\ \hline
\multicolumn{1}{|l|}{serpent}                                                           & \multicolumn{1}{c|}{$\surd$}  & $\times$ & \multicolumn{1}{c|}{2}      & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{2}      & 0.07    \\ \hline
\multicolumn{1}{|l|}{serpent}                                                           & \multicolumn{1}{c|}{$\surd$}  & $\surd$  & \multicolumn{1}{c|}{3}      & \multicolumn{1}{c|}{0.08}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.08}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.09}   & \multicolumn{1}{c|}{3}      & 0.09    \\ \hline
\multicolumn{1}{|l|}{sipma91}                                                           & \multicolumn{1}{c|}{$\times$} & $\times$ & \multicolumn{1}{c|}{2}      & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{2}      & 0.08    \\ \hline
\multicolumn{1}{|l|}{sipma91}                                                           & \multicolumn{1}{c|}{$\surd$}  & $\times$ & \multicolumn{1}{c|}{1}      & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{1}     & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{1}     & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{1}      & 0.06    \\ \hline
\multicolumn{1}{|l|}{sipma91}                                                           & \multicolumn{1}{c|}{$\surd$}  & $\surd$  & \multicolumn{1}{c|}{2}      & \multicolumn{1}{c|}{0.08}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.08}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.09}   & \multicolumn{1}{c|}{2}      & 0.08    \\ \hline
\multicolumn{1}{|l|}{sipmabubble}                                                       & \multicolumn{1}{c|}{$\times$} & $\times$ & \multicolumn{1}{c|}{3}      & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{3}      & 0.08    \\ \hline
\multicolumn{1}{|l|}{sipmabubble}                                                       & \multicolumn{1}{c|}{$\surd$}  & $\times$ & \multicolumn{1}{c|}{3}      & \multicolumn{1}{c|}{0.08}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.08}   & \multicolumn{1}{c|}{3}      & 0.08    \\ \hline
\multicolumn{1}{|l|}{sipmabubble}                                                       & \multicolumn{1}{c|}{$\surd$}  & $\surd$  & \multicolumn{1}{c|}{3}      & \multicolumn{1}{c|}{0.08}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.08}   & \multicolumn{1}{c|}{3}      & 0.08    \\ \hline
\multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}sipma\\ mergesort\end{tabular}}         & \multicolumn{1}{c|}{$\times$} & $\times$ & \multicolumn{1}{c|}{$\times$}  & \multicolumn{1}{c|}{213.99} & \multicolumn{1}{c|}{$\times$} & \multicolumn{1}{c|}{185.24} & \multicolumn{1}{c|}{$\times$} & \multicolumn{1}{c|}{183.39} & \multicolumn{1}{c|}{$\times$*} & $\times$*  \\ \hline
\multicolumn{1}{|l|}{speedDis1}                                                         & \multicolumn{1}{c|}{$\times$} & $\times$ & \multicolumn{1}{c|}{$\times$}  & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{$\times$} & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{4}     & \multicolumn{1}{c|}{0.09}   & \multicolumn{1}{c|}{4}      & 0.19    \\ \hline
\multicolumn{1}{|l|}{speedDis2}                                                         & \multicolumn{1}{c|}{$\times$} & $\times$ & \multicolumn{1}{c|}{$\times$}  & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{$\times$} & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{4}     & \multicolumn{1}{c|}{0.09}   & \multicolumn{1}{c|}{4}      & 0.10    \\ \hline
\multicolumn{1}{|l|}{speedFails1}                                                       & \multicolumn{1}{c|}{$\times$} & $\times$ & \multicolumn{1}{c|}{2}      & \multicolumn{1}{c|}{0.05}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.05}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.05}   & \multicolumn{1}{c|}{2}      & 0.06    \\ \hline
\multicolumn{1}{|l|}{speedFails1}                                                       & \multicolumn{1}{c|}{$\surd$}  & $\times$ & \multicolumn{1}{c|}{2}      & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.05}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{2}      & 0.06    \\ \hline
\multicolumn{1}{|l|}{speedFails1}                                                       & \multicolumn{1}{c|}{$\surd$}  & $\surd$  & \multicolumn{1}{c|}{2}      & \multicolumn{1}{c|}{0.05}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.05}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.05}   & \multicolumn{1}{c|}{2}      & 0.06    \\ \hline
\multicolumn{1}{|l|}{speedFails2}                                                       & \multicolumn{1}{c|}{$\times$} & $\times$ & \multicolumn{1}{c|}{$\times$}  & \multicolumn{1}{c|}{0.05}   & \multicolumn{1}{c|}{$\times$} & \multicolumn{1}{c|}{0.05}   & \multicolumn{1}{c|}{$\times$} & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{$\times$}  & 0.07    \\ \hline
\multicolumn{1}{|l|}{speedFails2}                                                       & \multicolumn{1}{c|}{$\surd$}  & $\times$ & \multicolumn{1}{c|}{$\times$}  & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{$\times$} & \multicolumn{1}{c|}{0.05}   & \multicolumn{1}{c|}{$\times$} & \multicolumn{1}{c|}{0.08}   & \multicolumn{1}{c|}{$\times$}  & 0.17    \\ \hline
\multicolumn{1}{|l|}{speedFails2}                                                       & \multicolumn{1}{c|}{$\surd$}  & $\surd$  & \multicolumn{1}{c|}{$\times$}  & \multicolumn{1}{c|}{0.05}   & \multicolumn{1}{c|}{$\times$} & \multicolumn{1}{c|}{0.05}   & \multicolumn{1}{c|}{$\times$} & \multicolumn{1}{c|}{0.08}   & \multicolumn{1}{c|}{$\times$}  & 0.18    \\ \hline
\multicolumn{1}{|l|}{speedFails4}                                                       & \multicolumn{1}{c|}{$\times$} & $\times$ & \multicolumn{1}{c|}{$\times$}  & \multicolumn{1}{c|}{0.05}   & \multicolumn{1}{c|}{$\times$} & \multicolumn{1}{c|}{0.05}   & \multicolumn{1}{c|}{$\times$} & \multicolumn{1}{c|}{0.09}   & \multicolumn{1}{c|}{$\times$}  & 0.30    \\ \hline
\multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}speedNested\\ Multiple\end{tabular}}    & \multicolumn{1}{c|}{$\times$} & $\times$ & \multicolumn{1}{c|}{3}      & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{3}      & 0.07    \\ \hline
\multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}speedNested\\ Multiple\end{tabular}}    & \multicolumn{1}{c|}{$\surd$}  & $\times$ & \multicolumn{1}{c|}{3}      & \multicolumn{1}{c|}{0.08}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{3}      & 0.07    \\ \hline
\multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}speedNested\\ Multiple\end{tabular}}    & \multicolumn{1}{c|}{$\surd$}  & $\surd$  & \multicolumn{1}{c|}{3}      & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{3}      & 0.07    \\ \hline
\multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}speedNested\\ MultipleDep\end{tabular}} & \multicolumn{1}{c|}{$\times$} & $\times$ & \multicolumn{1}{c|}{3}      & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{3}      & 0.07    \\ \hline
\multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}speedNested\\ MultipleDep\end{tabular}} & \multicolumn{1}{c|}{$\surd$}  & $\times$ & \multicolumn{1}{c|}{3}      & \multicolumn{1}{c|}{0.09}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{3}      & 0.07    \\ \hline
\multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}speedNested\\ MultipleDep\end{tabular}} & \multicolumn{1}{c|}{$\surd$}  & $\surd$  & \multicolumn{1}{c|}{3}      & \multicolumn{1}{c|}{0.08}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.08}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.08}   & \multicolumn{1}{c|}{3}      & 0.08    \\ \hline
\multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}speedSimple\\ Multiple\end{tabular}}    & \multicolumn{1}{c|}{$\times$} & $\times$ & \multicolumn{1}{c|}{$\times$}  & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{$\times$} & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{4}     & \multicolumn{1}{c|}{0.08}   & \multicolumn{1}{c|}{4}      & 0.10    \\ \hline
\multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}speedSimple\\ MultipleDep\end{tabular}} & \multicolumn{1}{c|}{$\times$} & $\times$ & \multicolumn{1}{c|}{$\times$}  & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{$\times$} & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{4}     & \multicolumn{1}{c|}{0.09}   & \multicolumn{1}{c|}{4}      & 0.10    \\ \hline
\multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}speedSingle\\ Single\end{tabular}}      & \multicolumn{1}{c|}{$\times$} & $\times$ & \multicolumn{1}{c|}{2}      & \multicolumn{1}{c|}{0.05}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.05}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{2}      & 0.06    \\ \hline
\multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}speedSingle\\ Single\end{tabular}}      & \multicolumn{1}{c|}{$\surd$}  & $\times$ & \multicolumn{1}{c|}{2}      & \multicolumn{1}{c|}{0.10}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.05}   & \multicolumn{1}{c|}{2}      & 0.06    \\ \hline
\multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}speedSingle\\ Single\end{tabular}}      & \multicolumn{1}{c|}{$\surd$}  & $\surd$  & \multicolumn{1}{c|}{2}      & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{2}      & 0.06    \\ \hline
\multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}speedSingle\\ Single2\end{tabular}}     & \multicolumn{1}{c|}{$\times$} & $\times$ & \multicolumn{1}{c|}{2}      & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{2}      & 0.06    \\ \hline
\multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}speedSingle\\ Single2\end{tabular}}     & \multicolumn{1}{c|}{$\surd$}  & $\times$ & \multicolumn{1}{c|}{2}      & \multicolumn{1}{c|}{0.08}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{2}      & 0.07    \\ \hline
\multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}speedSingle\\ Single2\end{tabular}}     & \multicolumn{1}{c|}{$\surd$}  & $\surd$  & \multicolumn{1}{c|}{$\times$}  & \multicolumn{1}{c|}{0.08}   & \multicolumn{1}{c|}{$\times$} & \multicolumn{1}{c|}{0.08}   & \multicolumn{1}{c|}{5}     & \multicolumn{1}{c|}{0.17}   & \multicolumn{1}{c|}{5}      & 1.79    \\ \hline
\multicolumn{1}{|l|}{speedpldi2}                                                        & \multicolumn{1}{c|}{$\times$} & $\times$ & \multicolumn{1}{c|}{2}      & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.05}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{2}      & 0.06    \\ \hline
\multicolumn{1}{|l|}{speedpldi2}                                                        & \multicolumn{1}{c|}{$\surd$}  & $\times$ & \multicolumn{1}{c|}{2}      & \multicolumn{1}{c|}{0.08}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.05}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{2}      & 0.06    \\ \hline
\multicolumn{1}{|l|}{speedpldi2}                                                        & \multicolumn{1}{c|}{$\surd$}  & $\surd$  & \multicolumn{1}{c|}{2}      & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{2}      & 0.07    \\ \hline
\multicolumn{1}{|l|}{speedpldi3}                                                        & \multicolumn{1}{c|}{$\times$} & $\times$ & \multicolumn{1}{c|}{$\times$}  & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{3}      & 0.07    \\ \hline
\multicolumn{1}{|l|}{speedpldi3}                                                        & \multicolumn{1}{c|}{$\surd$}  & $\times$ & \multicolumn{1}{c|}{$\times$}  & \multicolumn{1}{c|}{0.08}   & \multicolumn{1}{c|}{$\times$} & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{4}     & \multicolumn{1}{c|}{0.10}   & \multicolumn{1}{c|}{4}      & 0.18    \\ \hline
\multicolumn{1}{|l|}{speedpldi3}                                                        & \multicolumn{1}{c|}{$\surd$}  & $\surd$  & \multicolumn{1}{c|}{3}      & \multicolumn{1}{c|}{0.08}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.08}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.08}   & \multicolumn{1}{c|}{3}      & 0.09    \\ \hline
\multicolumn{1}{|l|}{speedpldi4}                                                        & \multicolumn{1}{c|}{$\times$} & $\times$ & \multicolumn{1}{c|}{2}      & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.05}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{2}      & 0.06    \\ \hline
\multicolumn{1}{|l|}{speedpldi4}                                                        & \multicolumn{1}{c|}{$\surd$}  & $\times$ & \multicolumn{1}{c|}{2}      & \multicolumn{1}{c|}{0.09}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.05}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{2}      & 0.06    \\ \hline
\multicolumn{1}{|l|}{speedpldi4}                                                        & \multicolumn{1}{c|}{$\surd$}  & $\surd$  & \multicolumn{1}{c|}{2}      & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{2}      & 0.06    \\ \hline
\multicolumn{1}{|l|}{terminate}                                                         & \multicolumn{1}{c|}{$\times$} & $\times$ & \multicolumn{1}{c|}{2}      & \multicolumn{1}{c|}{0.05}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.05}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{2}      & 0.06    \\ \hline
\multicolumn{1}{|l|}{terminate}                                                         & \multicolumn{1}{c|}{$\surd$}  & $\times$ & \multicolumn{1}{c|}{2}      & \multicolumn{1}{c|}{0.08}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.05}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{2}      & 0.06    \\ \hline
\multicolumn{1}{|l|}{terminate}                                                         & \multicolumn{1}{c|}{$\surd$}  & $\surd$  & \multicolumn{1}{c|}{2}      & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{2}      & 0.06    \\ \hline
\multicolumn{1}{|l|}{unperfect}                                                         & \multicolumn{1}{c|}{$\times$} & $\times$ & \multicolumn{1}{c|}{3}      & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.08}   & \multicolumn{1}{c|}{3}      & 0.07    \\ \hline
\multicolumn{1}{|l|}{unperfect}                                                         & \multicolumn{1}{c|}{$\surd$}  & $\times$ & \multicolumn{1}{c|}{3}      & \multicolumn{1}{c|}{0.10}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.08}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.08}   & \multicolumn{1}{c|}{3}      & 0.08    \\ \hline
\multicolumn{1}{|l|}{unperfect}                                                         & \multicolumn{1}{c|}{$\surd$}  & $\surd$  & \multicolumn{1}{c|}{$\times$}  & \multicolumn{1}{c|}{0.09}   & \multicolumn{1}{c|}{$\times$} & \multicolumn{1}{c|}{0.10}   & \multicolumn{1}{c|}{$\times$} & \multicolumn{1}{c|}{0.34}   & \multicolumn{1}{c|}{$\times$}  & 473.42  \\ \hline
\multicolumn{1}{|l|}{wcet0}                                                             & \multicolumn{1}{c|}{$\times$} & $\times$ & \multicolumn{1}{c|}{2}      & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.08}   & \multicolumn{1}{c|}{2}      & 0.06    \\ \hline
\multicolumn{1}{|l|}{wcet0}                                                             & \multicolumn{1}{c|}{$\surd$}  & $\times$ & \multicolumn{1}{c|}{2}      & \multicolumn{1}{c|}{0.09}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{2}      & 0.07    \\ \hline
\multicolumn{1}{|l|}{wcet0}                                                             & \multicolumn{1}{c|}{$\surd$}  & $\surd$  & \multicolumn{1}{c|}{2}      & \multicolumn{1}{c|}{0.08}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.08}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.08}   & \multicolumn{1}{c|}{2}      & 0.10    \\ \hline
\multicolumn{1}{|l|}{wcet1}                                                             & \multicolumn{1}{c|}{$\times$} & $\times$ & \multicolumn{1}{c|}{2}      & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{2}      & 0.06    \\ \hline
\multicolumn{1}{|l|}{wcet1}                                                             & \multicolumn{1}{c|}{$\surd$}  & $\times$ & \multicolumn{1}{c|}{2}      & \multicolumn{1}{c|}{0.11}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{2}      & 0.07    \\ \hline
\multicolumn{1}{|l|}{wcet1}                                                             & \multicolumn{1}{c|}{$\surd$}  & $\surd$  & \multicolumn{1}{c|}{2}      & \multicolumn{1}{c|}{0.08}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.09}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{2}      & 0.08    \\ \hline
\multicolumn{1}{|l|}{wcet2}                                                             & \multicolumn{1}{c|}{$\times$} & $\times$ & \multicolumn{1}{c|}{2}      & \multicolumn{1}{c|}{0.05}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.05}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{2}      & 0.06    \\ \hline
\multicolumn{1}{|l|}{wcet2}                                                             & \multicolumn{1}{c|}{$\surd$}  & $\times$ & \multicolumn{1}{c|}{2}      & \multicolumn{1}{c|}{0.09}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{2}      & 0.06    \\ \hline
\multicolumn{1}{|l|}{wcet2}                                                             & \multicolumn{1}{c|}{$\surd$}  & $\surd$  & \multicolumn{1}{c|}{2}      & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{2}      & 0.06    \\ \hline
\multicolumn{1}{|l|}{while2}                                                            & \multicolumn{1}{c|}{$\times$} & $\times$ & \multicolumn{1}{c|}{3}      & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{3}      & 0.07    \\ \hline
\multicolumn{1}{|l|}{while2}                                                            & \multicolumn{1}{c|}{$\surd$}  & $\times$ & \multicolumn{1}{c|}{3}      & \multicolumn{1}{c|}{0.11}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{3}      & 0.07    \\ \hline
\multicolumn{1}{|l|}{while2}                                                            & \multicolumn{1}{c|}{$\surd$}  & $\surd$  & \multicolumn{1}{c|}{3}      & \multicolumn{1}{c|}{0.07}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.08}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.08}   & \multicolumn{1}{c|}{3}      & 0.08    \\ \hline
\multicolumn{1}{|l|}{wise}                                                              & \multicolumn{1}{c|}{$\times$} & $\times$ & \multicolumn{1}{c|}{$\times$}  & \multicolumn{1}{c|}{0.05}   & \multicolumn{1}{c|}{$\times$} & \multicolumn{1}{c|}{0.05}   & \multicolumn{1}{c|}{$\times$} & \multicolumn{1}{c|}{0.09}   & \multicolumn{1}{c|}{$\times$}  & 0.29    \\ \hline
\multicolumn{1}{|l|}{counterexStr1}                                                     & \multicolumn{1}{c|}{$\times$} & $\surd$  & \multicolumn{1}{c|}{N/A} & \multicolumn{1}{c|}{N/A} & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.08}   & \multicolumn{1}{c|}{3}     & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{3}      & 0.18    \\ \hline
\multicolumn{1}{|l|}{counterexStr2}                                                     & \multicolumn{1}{c|}{$\times$} & $\surd$  & \multicolumn{1}{c|}{$\times$}  & \multicolumn{1}{c|}{0.06}   & \multicolumn{1}{c|}{$\times$} & \multicolumn{1}{c|}{0.10}   & \multicolumn{1}{c|}{4}     & \multicolumn{1}{c|}{0.13}   & \multicolumn{1}{c|}{4}      & 0.36    \\ \hline
\end{longtable}
